Our Galaxy's youngest disc

We investigate the structure of our Galaxy's young stellar disc by fitting the distribution functions (DFs) of a new family to five-dimensional Gaia data for a sample of $47\,000$ OB stars. Tests of the fitting procedure show that the young disc's DF would be strongly constrained by Gaia data if the distribution of Galactic dust were accurately known. The DF that best fits the real data accurately predicts the kinematics of stars at their observed locations, but it predicts the spatial distribution of stars poorly, almost certainly on account of errors in the best-available dust map. We argue that dust models could be greatly improved by modifying the dust model until the spatial distribution of stars predicted by a DF agreed with the data. The surface density of OB stars is predicted to peak at $R\simeq5.5\mbox{kpc}$, slightly outside the reported peak in the surface density of molecular gas; we suggest that the latter radius may have been under-estimated through the use of poor kinematic distances. The velocity distributions predicted by the best-fit DF for stars with measured line-of-sight velocities $v_\parallel$ reveal that the outer disc is disturbed at the level of 10 $\mbox{km}~\mbox{s}^{-1}$ in agreement with earlier studies, and that the measured values of $v_\parallel$ have significant contributions from the orbital velocities of binaries. Hence the outer disc is colder than it is sometimes reported to be.

==> notes <==
Fig 2
I suggest we break this into 2 figs. The top 2 panels as a single {figure*} and
the lower four compacted into a {figure}. In that I'd like l=45 and l=225 in
top row and l=135 and 315 in the lower row. In each row both left and right
panels would have the same A scale, so we can have touching panels. If you
send me that data, I'm happy to do the plots.

-------------------done-----------------------


Fig 4 
I think the lower panel should look more like the upper panel. That is,
it should be illustrating that by varying both p_z and J_{z0} we can have all
3 curves overlapping as they pass through the pea of the data.

-------------------------------done--------------------------------------

Figs 6,7,8,9
I think we can compress these into {figure} rather than {figure*} by using
touching panels. We don't need "Bin 1," etc just "r=.." I think all V scales
can be (-100,100) for Vb or (-300,300) for V\ell

-------------------------done----------------------------------



Fig 11
We need only the right panel   -----------done-----------------

Fig 12
Can (i) we change the vertical scale so the curve comes nearer the top; (ii)
move the blue points up so they scatter around the curve; (iii) remove the
vertical lines?        ------------------done-------------------------

Fig 13
I think we should delete the broken curves & change vertical scale to extend
only to 80 km/s    --------------done----------------------

Fig 14
Remove the vertical lines and change the vertical scale to 80 km/s  -----------------done--------

Fig 17 We can make this a {figure} rather than {figure*} by using touching
panels for the top four panels and separately for the bottom 2 panels.


------------------------done----------------------------------------



draw a new circular velocity fig. and add a tabel reporting mass of the disc and the density in solar radius at z=0 and z=1

The disk mass and rho at solar radius
Disk total mass=5.48235e+10 Msun, rho(Rsolar,z=0)=0.0949925, rho(Rsolar,z=1kpc)=0.00496985 Msun/pc^3
-----------------------done-------------------------------


add a paragrahp telling about the wrong dust model



